Self-Perception Versus Objective Driving Behavior: Subject Study of Lateral Vehicle Guidance

Advancements in technology are steering attention toward creating comfortable and acceptable driving characteristics in autonomous vehicles. Ensuring a safe and comfortable ride experience is vital for the widespread adoption of autonomous vehicles, as mismatches in driving styles between humans and autonomous systems can impact passenger confidence. Current driving functions have fixed parameters, and there is no universally agreed-upon driving style for autonomous vehicles. Integrating driving style preferences into automated vehicles may enhance acceptance and reduce uncertainty, expediting their adoption. A controlled vehicle study (N = 62) was conducted with a variety of German participants to identify the individual lateral driving behavior of human drivers, specifically emphasizing rural roads. We introduce novel indicators for assessing stationary and transient curve negotiation, directly applicable in developing personalized lateral driving functions. To assess the predictability of these indicators using self-reports, we introduce the MDSI-DE, the German version of the Multidimensional Driving Style Inventory. The correlation analysis between MDSI factor scores and proposed indicators showed modest but significant associations, primarily with acceleration and jerk statistics while the in-depth lateral driving behavior turned out to be highly driver-heterogeneous. The dataset including the anonymized socio-demographics and questionnaire responses, the raw vehicle measurements including labels, and the derived driving behavior indicators are publicly available at https://www.kaggle.com/datasets/jhaselberger/spodb-subject-study-of-lateral-vehicle-guidance.

==> nomenclature.tex <==
% nomenclature

==> sections/methodology/method_lit_references.tex <==
\subsection{Lit References for Methodology}

% \subsubsection{General}
% \jRef{
% \begin{itemize}
%     % \item \cite{amado2014accurately}: Participants were interviewed before arrival to verify eligibility, and were given an appointment. Upon arrival they signed an informed consent form, completed the driver information form and were escorted by two research associate expert observers (both were experienced drivers education instructors). They were given information about the driving route, and were told to drive naturally, as usual. One of the observers sat at the rear, provided directions, and otherwise remained silent during the driving session. The other observer sat at the back, and they both used an observation form for data collection.
%     % \item \cite{amado2014accurately}: Data was collected on a 45 km route in izmir, consisting of diverse road types: inner city road, two way road, single-track road, highway, crossroad, underground tunnel, etc. First 10 min of driving was not recorded in order to allow adaptation to the vehicle, and then approximately 80 min of driving was recorded.
%     % \item what was done after the ride?
%     % \item \cite{van2018relation}: focus on speed, acceleration ... as these measures (1) can be gained directly from the vehicle and (2) be measured continuously.
%     % \item \cite{van2018relation}: A related measure is jerk, which is defined as the rate of change in acceleration or deceleration, and represents how smooth people drive on straight road segments. Braking more abruptly, accelerating faster and driving more irregularly result in a higher average jerk compared to drivers who decelerate and accelerate more smoothly and maintain a more stable speed.
%     % \item Jerk has shown to be effective in the classification of driving styles. Calm drivers tend to anticipate more on other road users’ movements and traffic lights, resulting in less abrupt braking \cite{murphey2009driver}
%     \item \cite{just2008decrease}: increases in lane position variability are indicative of distracted driving and may therewith be associated with dissociative driving.
%     % \item The use of a driving simulator has several advantages over the use of an instrumented vehicle on public roads \cite{helman2015validation}
%     % \item driving simulator provides more control and consistency among different participants and allows eliciting particular behaviours in situations that may be difficult to realise, unsafe or impractical in the real world \cite{reimer2006using}
%     % \item \cite{van2018relation}: driving in a driving simulator enables risky behaviour or situations without real threats for the drivers themselves, giving participants the opportunity to practice tendencies that are difficult to practice on the roads, because of the constraints on real-life behaviour.
%     % \item \cite{van2018relation}: use of a driving simulator may also have disadvantages that may affect the observed behaviour
%     % \item \cite{van2018relation}: the fidelity of the simulator may influence the perception of the driver
%     % \item \cite{van2018relation}:  some drivers interpret events and situations in a simulator as less dangerous compared to the same type of events and situations encountering on the road \cite{helman2015validation}
%     % \item \cite{van2018relation}: The study involved two tasks, filling in the MDSI questionnaire and driving in the driving simulator. Participants were asked to complete the MDSI questionnaire beforehand at home and to subscribe for a timeslot to participate in the driving simulator part of this study. The driving session was concluded with a brief interview.
%     % \item The questionnaire assesses six factors: Angry driving (7 items, Cronbach’s alpha .81), Risky driving (5 items, Cronbach’s alpha .83) ...
%     % \item \cite{van2018relation}: uses sum scores by factors to for the driving style scores
%     % \item The translation of the MDSI aimed at preserving the meaning of the questions instead of a literal translation
%     % \item \cite{van2018relation}: Next to the questions of the MDSI, the questionnaire also contained questions concerning demographic data such as gender and age and driving history such as the amount of time being in possession of a driver’s license and the annual number of kilometres driven.
%     % \item  Participants were instructed to drive in the simulator as they would normally drive in their own vehicle.
%     % \item During the sessions, the researcher sat behind a partition monitoring the participant and scenario through a video connection and marked remarkable behaviours in the video recording.
%     \item invitation to participate was also placed on a local website and in a newsletter of a trade union. The invitation consisted of a short explanation of the current study and provided a link to fill in the online questionnaire in advance of the simulator study. A second link allowed the participants to choose a suitable timeslot for driving in the driving simulator. 
%     % \item \cite{van2018relation}: Fifty-seven males (78.1\%) and sixteen females (21.9\%)
%     % \item \cite{helman2015validation}: The exploitation of results from simulator studies depends on the extent to which behaviours observed in the study represent behaviours in an equivalent real world situation
%     % \item \cite{helman2015validation}: participants will be aware that they are driving a simulator and that a collision in the simulator will not result in injury to themselves or third parties.
%     % \item Simulator sickness or simulator adaptation syndrome (SAS)\cite{mollenhauer2004simulator} can influence the results of driving experiment!
%     % \item \cite{helman2015validation}: participants may attempt to adopt a driving style that minimises the symptoms of simulator sickness (e.g. avoiding rapid changes in speed or direction) rather than in a manner representative of their real world driving.
%     % \item \cite{helman2015validation}: Since, the participants were told to drive as they normally would, and were generally free to choose their own speed on each bend (data points were removed where video showed that leading traf fi c was ‘ holding up ’ participants) we make the assumption that the data re fl ect to some extent the usual driving behaviour of the participants
%     % \item \cite{helman2015validation}: since the participant numbers in our existing dataset precludes any further factor analysis to check factor structure, we restrict ourselves to using the broad factor structure of the scale suggested by XYZ
%     % \item \cite{helman2015validation}: sample was split equally between four age groups (17 – 26, 34 – 50, 60 – 75, 75+).
%     % \item \cite{helman2015validation}: Using objective behavioural data such as those from instrumented vehicles and from simulators in validating self-report measures helps to overcome much of the criticism that has been aimed at those measures in the literature (especially regarding common-method variance).
% \end{itemize}
% }

% \subsubsection{Questionnaire}
% \jRef{
% \begin{itemize}
%     % \item \cite{herrero2021people}: The internal consistency reported values (Cronbach’s  alpha) are referred to the current sample
%     % \item \cite{herrero2021people} The MDSI (Taub man-Ben-Ari et al., 2004) is a self-report for measuring the ways drivers choose to drive or habitually drive.
%     % \item The whole questionnaire is composed of N questions distributed to the M factors: X (Cronbach's alpha = 0.000)...
%     % \item Questions were asked using online tool 
%     % \item how the Participants were gained?
%     % \item \cite{herrero2021people} The questionnaire began with an information sheet in which the goals of the study and the approximate length of the questionnaire were explained. The requirement of both having a valid type B driving license (the legal requirement for regular cars, according to the Spanish driving regulations) at the moment of completing the questionnaires and driving at least once a week was explained. At the same time, the individual’s anonymity and voluntary status were assured, and the participant had to click at the bottom of this first page accepting the conditions to take part in the study. It was taken as the signature for the study’s informed consent. This study is a part of an extensive project that was approved by the Research Ethics Board of the European University of the Atlantic.
%     % \item \cite{herrero2021people} Finally, there were no missing data in the questionnaires, as every item had to be answered to be able to complete and send off the poll, and those participants who indicated driving 0 times per week were removed from the final data base. 
%     % \item \cite{van2018relation}: MDSI adapted items from several other existing surveys, such as the Driver Behaviour Inventory (DBI) \cite{gulian1989dimensions}, the Driver Behaviour Questionnaire (DBQ) \cite{reason1990errors}, the Driver Behaviour Questionnaire \cite{furnham1993personality} and the Driver Style Questionnaire (DSQ) \cite{french1993decision} CHECK IF THE CITE FOR DSQ IS CORRECT!
%     \item \cite{van2018relation}: A modified version of the MDSI questionnaire was used in the current study, which resulted from a validation study with mainly Dutch and Belgian respondents, and which contains 37 items that distinguish six of the original eight driving styles \cite{van2015measuring}
% \end{itemize}
% }

==> sections/related/lit_references.tex <==
% \jRef{
%     \begin{itemize}
         
%     \end{itemize}
% }

==> tables/__latexindent_temp.tex <==
\begin{table}[]
    \caption{\small{XYZ data split into Women(N=17) and Men (N=45).}}
    \centering
    \begin{tabular}{lllllll}
    \hline
    Car usage            &        &    &  & Anual milage       &        &    \\ \cline{1-3} \cline{5-7} 
    Response             & Gender & N  &  & Response           & Gender & N  \\ \hline
    Daily                & female & 9  &  & 0 - 5000           & female & 4  \\
                         & male   & 21 &  &                    & male   & 3  \\
    Several times a week & female & 7  &  & 5000 - 10000       & female & 4  \\
                         & male   & 16 &  &                    & male   & 9  \\
    Weekly               & female & 0  &  & 10000 -20000       & female & 9  \\
                         & male   & 5  &  &                    & male   & 19 \\
    Few times a month    & female & 1  &  & 20000 - 30000      & female & 0  \\
                         & male   & 3  &  &                    & male   & 12 \\
                         &        &    &  & \textgreater 30000 & female & 0  \\
                         &        &    &  &                    & male   & 2  \\ \hline
    \end{tabular}
    \label{tab:participants02}
    \end{table}
